AI-based Question Answering Assistance for Analyzing Natural-language Requirements

By virtue of being prevalently written in natural language (NL), requirements are prone to various defects, e.g., inconsistency and incompleteness. As such, requirements are frequently subject to quality assurance processes. These processes, when carried out entirely manually, are tedious and may further overlook important quality issues due to time and budget pressures. In this paper, we propose QAssist -- a question-answering (QA) approach that provides automated assistance to stakeholders, including requirements engineers, during the analysis of NL requirements. Posing a question and getting an instant answer is beneficial in various quality-assurance scenarios, e.g., incompleteness detection. Answering requirements-related questions automatically is challenging since the scope of the search for answers can go beyond the given requirements specification. To that end, QAssist provides support for mining external domain-knowledge resources. Our work is one of the first initiatives to bring together QA and external domain knowledge for addressing requirements engineering challenges. We evaluate QAssist on a dataset covering three application domains and containing a total of 387 question-answer pairs. We experiment with state-of-the-art QA methods, based primarily on recent large-scale language models. In our empirical study, QAssist localizes the answer to a question to three passages within the requirements specification and within the external domain-knowledge resource with an average recall of 90.1% and 96.5%, respectively. QAssist extracts the actual answer to the posed question with an average accuracy of 84.2%. Keywords: Natural-language Requirements, Question Answering (QA), Language Models, Natural Language Processing (NLP), Natural Language Generation (NLG), BERT, T5.

==> sections/dataset.tex <==

\section{Question Generation from Requirements}\label{sec:nlg}
%overgenerate-and-rank approach
Though many QA datasets are publicly available, none of them is tailored to address the needs of RE community. Therefore, as a prerequisite to developing a QA assistant to requirements engineers, we had to first create a dataset. We will refer to our dataset as \emph{JAWAB}, standing for ``Joint question-AnsWer pairs for Acquiring Background''. 
In this section, we first outline the goals for JAWAB, and then the method we used to generate different types of \emph{question-answer (i.e., q-a) pairs} in JAWAB.

\subsection{Desiderata}

To create a dataset that enables developing a QA assistance for requirements engineers, we posit the following desiderata specific to JAWAB: 

\noindent (1) Content-based q-a pairs. Unlike existing datasets in RE which cover questions related to RE tasks, e.g., change impact analysis, JAWAB covers content-based questions, i.e., clarification questions that can be useful for the engineer to acquire necessary background or missing details.


\noindent (2) RS snippets triggering questions should not necessarily contain the answer. To  provide a meaningful assistance, the answers to the questions raised by the requirements engineers are expected to be in distant parts of the same documents, i.e., outside the range of the engineer's current review, or outside the document, e.g., definitions or further details related to domain knowledge but not explicitly mentioned in the RS. Unlike conventional reading comprehension datasets, JAWAB does not cover q-a pairs originating from snippets that have no relatedness to any other snippet in the RS. 

\noindent (3) Domain-based questions should be possible.  JAWAB covers domain-based questions, i.e., questions whose answers are not in the RS. Assuming that a domain-specific corpus is available for each RS, we generate questions from the RS whose answers are mined in the corpus. 


\subsection{Dataset Creation}

\subsubsection{Document-based QG}
\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{figs/question-generation.pdf}
  \caption{Document-based Question Generation Method}
  \label{fig:qg-overview}
\end{figure*}

\sectopic{Preprocessing} 
In the first step we preprocess the input RS applying a standard NLP pipeline (e.g., tokenizer, lemmatizer, NER), and dismissing irrelevant parts and sections (Introduction, Table of contents, Titles, sub-titles, etc).

\sectopic{Context Selection}
We define the context as paragraphs of maximum length of 512 tokens (if a paragraph is longer than the max context size, then it is split into multiple contexts while keeping a one sentence overlap to ensure context continuity). In requirements engineering we are interested to generate questions where the answer if found in other contexts rather then having a question that can only be asked and answered from the same context. So in order to filter out isolated and disconnected context we drop contexts that does not have any cross-context similarity.

\sectopic{Answer Selection}
In case of multi-choice questions, the answer is is selected using a combination of different approaches. Names entities and noun phrases are the most popular solutions for answer selection \cite{Ch:18}, but instead of selecting all noun phrases we select top-K frequent ones. We also use key phrases extraction and ranking \cite{Willis:19,Awan:21}. The extracted answer-sets (name entities, noun phrases and key phrases) are then passed to pair-wise similarity filter to remove isolated and out-of-the-context instances. %looking for citation
For full-sentence answer style we select all tokenized sentences from the context.

\sectopic{Question Generation}
Next, we apply multiple pretrained QG models trained on different datasets to generate different answer styles (i.e., Boolean, Multi-Choice, and Full Sentence). Then they generate multiple questions from the input context-answer pairs, the output can be considered as context-question-answer triplets.

The QG models we use are variants of T5-based sequence-to-sequence question generator that takes a context-answer pair as input and generates a question as an output. The models are trained on different QA datasets namely Quora Question pairs~\cite{Quora:18}, RACE~\cite{RACE:17}, CoQA~\cite{CoQA:19}, BoolQ~\cite{BoolQ:19}, SQUAD~\cite{SQUAD:16}, and MSMarco~\cite{MSMarco:16}.


\sectopic{Q-A Pair Evaluator}
To ensure the quality of our generated data, we evaluate the question-answer pairs using a dedicated classification model. This evaluation model is trained to rank question-answer pairs based on their quality.
For each input document we set the desired number of questions (n). This number is then split between the question-answer styles (e.g., $n = f + m + b$. The evaluation model selects top k-ranked questions from each type filling the fixed numbers.

We use two selection methods for Boolean questions. In the first one, we simply select top k-ranked Boolean generated questions using the QA evaluator. The second method consists of using unsupervised learning to get more diversified questions. The set of Boolean questions is then clustered into k-cluster (k is the desired number from this phase) and the top ranked question is selected from each cluster. In our work, we take the union for both methods' results.


%for generating the question-answer pairs, we use T5 and Questgen 
% the two models are variants of T which are trained on different datasets, and enable generating diverse types of questions
%for evaluating and ranking the question-answer pairs, we use BERT 

\subsubsection{Domain-based QG}

\sectopic{Natural Language Processing (NLP) Pipeline. }
In our work, we apply an NLP pipeline composed of seven modules: 
(1)~\textit{tokenizer} for splitting the text into tokens; (2)~\textit{sentence splitter} for breaking up the text into individual sentences; (3)~\textit{part-of-speech (POS) tagger} for assigning a POS tag, e.g., noun, verb or pronoun, to each token in each sentence; (4)~\textit{lemmatizer} for identifying the canonical form (lemma) of each token, e.g., the lemma for ``playing'' is ``play''; (5)~\textit{constituency parser} for identifying the structural units of sentences, e.g., NPs; and  (6)~\textit{named entity recognizer} for identifying the named entities in sentences. (7)~\textit{stop-words remover} to remove the most common English words.

\sectopic{Domain-specific keywords extraction}
We extract name entities and noun phrases from the input documents. These keywords are then ranked using term frequency–inverse domain frequency (TFIDmF) and. 


Batch-2
find keywords using TF IDF for domain specific

use Top-k

query Wikipedia - matching title with a sim value > X

After collecting articles (corpus generation) - we filter out the non-relevant content wise (sim value > Y) 

generate definition questions

we focused on summary paragraphs

Batch-3

Partition each article in Wikipedia 

Keep the contexts (partitions) in Wikipedia articles that contain at least one keyword

feed this in to QA generator and generate other type of questions 


==> sections/notation.tex <==
input question $q$ 

two question types $q_c$ (document based), $q_m$ (domain based)

Domain-specific corpus $\mathcal{D}$

relevant domain-related document $d_r \in \mathcal{D}$

input SRS 

(splitting) into a list of text passages ($t_i \in \mathcal{T}_c$ or $t_j \in \mathcal{T}_m$) originated from SRS or from $d_r \in \mathcal{D}$

[update] use one $\mathcal{T}$ and define it depending on where it comes

(step 4) the list of relevant text passages $\mathcal{R}$, such that $r_1 \ldots r_k$ are from $\mathcal{T}_c$ or $\mathcal{T}_m$

an answer to the question is $a$, the output contains $a_1 \ldots a_k$

In ground truth
$\langle q,a\rangle$ is a question-answer pair 
$\langle q_c,a_c\rangle$ is document-based and $\langle q_m,a_m\rangle$ is domain-based 



==> sections/running_example.tex <==
%%%%%%%Example 1%%%%%
R1. The spacecraft shall carry a science camera system as part of the scientific payload and a separate navigation camera system.

Question -> What is the function of science camera system?
Answer -> Not Found (because no additional information on science camera system) -- Incompleteness

%%%%%%%%EXample 2%%%%%%%

XX R1. The spacecraft shall carry a science camera system as part of the scientific payload and a separate navigation camera system.

R2 -- R2. The spacecraft shall carry a navigation camera system used only for the detection of the comet nucleus.

Rx. The navigation camera system as defined above shall also be used for asteroid detection, approach navigation and close fly-by tracking of the asteroid.

Question -> What is the function of navigation camera system?
Answer -> returns R2 and Rx (which have an inconsistency as R2 mentions only for detection of .. and Rx mentions also for...)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Example 3$%%%%

R1 -- R3. The wet mass of the spacecraft shall be computed at a regular basis, and not exceed 3004 kg. 

Question -> What is the wet mass of a spacecraft?
Answer from Wikipedia

